Koopman Based Trajectory Optimization with Mixed Boundaries

Trajectory optimization is a widely used tool in the design and control of dynamical systems. Typically, not only nonlinear dynamics, but also couplings of the initial and final condition through implicit boundary constraints render the optimization problem non-convex. This paper investigates how the Koopman operator framework can be utilized to solve trajectory optimization problems in a (partially) convex fashion. While the Koopman operator has already been successfully employed in model predictive control, the challenge of addressing mixed boundary constraints within the Koopman framework has remained an open question. We first address this issue by explaining why a complete convexification of the problem is not possible. Secondly, we propose a method where we transform the trajectory optimization problem into a bilevel problem in which we are then able to convexify the high-dimensional lower-level problem. This separation yields a low-dimensional upper-level problem, which could be exploited in global optimization algorithms. Lastly, we demonstrate the effectiveness of the method on two example systems: the mathematical pendulum and the compass-gait walker.

==> plots/resultsHO/HarmonicOscillatorPhaseSpace.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,1.00000,0.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.5\textwidth,
height=0.5\textwidth,
scale only axis,
xmin=-30,
xmax=30,
xlabel={$q$},
ymin=-30,
ymax=30,
ylabel={$\dot{q}$},
xmajorgrids,
ymajorgrids
]
\addplot [color=mycolor1, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
30	0\\
29.9396871935247	-1.89599466220109\\
29.7596652617197	-3.77118475146938\\
29.4614830646385	-5.61840156545118\\
29.0471395036024	-7.43063602865346\\
28.5190725800194	-9.20106405994891\\
27.8801468721002	-10.92307104725\\
27.1336394887774	-12.5902753468342\\
26.2832245652389	-14.1965507291033\\
25.3329563693066	-15.7360476970991\\
24.2872510924186	-17.2032136088502\\
23.1508674031898	-18.5928115395818\\
21.9288858454269	-19.8999378249499\\
20.6266871660362	-21.1200382317529\\
19.2499296614949	-22.2489227080038\\
17.8045256344302	-23.2827786697902\\
16.2966170543764	-24.2181827879957\\
14.7325505189425	-25.0521112436725\\
13.1188516134194	-25.7819484266327\\
11.4621987682866	-26.405494057632\\
9.76939671513847	-26.9209687203448\\
8.04734964224213	-27.3270177951451\\
6.30303415126098	-27.6227137924952\\
4.54347211663495	-27.8075570894927\\
2.77570354870284	-27.8814750787973\\
1.00675956088862	-27.844819744757\\
-0.756364459842153	-27.6983636870385\\
-2.50673538150913	-27.4432946174399\\
-4.23750845867744	-27.0812083607881\\
-5.94195297322476	-26.6141003959053\\
-7.6134772929295	-26.0443559775297\\
-9.24565325923962	-25.3747388847976\\
-10.8322398186216	-24.6083788464119\\
-12.3672058152076	-23.7487576969322\\
-13.844751866045	-22.7996943226978\\
-15.2593312440897	-21.7653284597433\\
-16.6056696981578	-20.6501034096593\\
-17.878784143342	-19.4587477426889\\
-19.0740001599004	-18.1962560604223\\
-20.1869682433016	-16.8678688932485\\
-21.2136787529677	-15.4790518102383\\
-22.150475512257	-14.0354738213605\\
-22.9940680173594	-12.5429851538712\\
-23.7415422180311	-11.0075944863554\\
-24.3903698384336	-9.43544572524275\\
-24.9384162117613	-7.8327944096611\\
-25.383946607817	-6.20598383123275\\
-25.7256310382075	-4.56142095585721\\
-25.9625475293606	-2.90555223466498\\
-26.0941838590959	-1.24483939116891\\
-26.1204377579925	0.414264728812614\\
-26.041615582269	2.06534015862947\\
-25.8584294703076	3.70202357886805\\
-25.5719930002965	5.31803176852071\\
-25.1838153717159	6.90718465734566\\
-24.695794138532	8.46342789935514\\
-24.1102065269831	9.98085488947705\\
-23.4296993757118	11.453728147791\\
-22.6572777407175	12.8764999983359\\
-21.7962922121472	14.2438324723112\\
-20.8504249943005	15.5506163685384\\
-19.8236748043838	16.7919894072994\\
-18.7203406494957	17.9633534171151\\
-17.5450045450461	19.0603904976577\\
-16.3025132412971	20.0790781057852\\
-14.9979590279539	21.0157030156455\\
-13.6366596897184	21.8668741078917\\
-12.2241376884361	22.6295339472777\\
-10.7660986499175	23.3009691122431\\
-9.2684092356815	23.8788192445345\\
-7.7370744817551	24.3610847914359\\
-6.17821468825751	24.7461334177738\\
-4.59804194479958	25.0327050695124\\
-3.00283637773407	25.2199156754403\\
-1.39892220599975	25.3072594781648\\
0.207356307290455	25.2946099903505\\
1.80965892025885	25.1822195768552\\
3.40167340760257	24.970717668112\\
4.97713939928354	24.6611076147667\\
6.52987197677158	24.2547621981871\\
8.05378494211539	23.7534178160121\\
9.54291367647561	23.1591673663678\\
10.9914375063932	22.4744518587607\\
12.3937014979801	21.7020507839214\\
13.7442376014015	20.8450712790261\\
15.0377850704565	19.9069361287403\\
16.2693100847597	18.8913706464075\\
17.4340245049531	17.8023884834227\\
18.527403694545	16.6442764183874\\
19.5452033453536	15.4215781810185\\
20.4834752471245	14.139077368972\\
21.3385819456802	12.8017795187378\\
22.1072102379291	11.4148933945471\\
22.7863834562054	9.98381156180722\\
23.3734724987059	8.51409031393187\\
23.8662055672318	7.01142902355588\\
24.2626765780098	5.48164899101364\\
24.5613522160453	3.93067186460695\\
24.7610776082385	2.36449770859158\\
24.8610805953487	0.789182795964583\\
24.8609745878174	-0.789182795964607\\
24.7607599954293	-2.36449770859159\\
24.5608242257968	-3.93067186460696\\
24.2619402516736	-5.48164899101364\\
23.8652637521224	-7.01142902355589\\
23.3723288375673	-8.51409031393187\\
22.7850423737318	-9.98381156180721\\
22.105676924387	-11.4148933945471\\
21.336862337689	-12.8017795187378\\
20.481576005664	-14.1390773689719\\
19.5431318310742	-15.4215781810184\\
18.5251679404693	-16.6442764183872\\
17.431633186664	-17.8023884834225\\
16.2667724881796	-18.8913706464074\\
15.0351110573324	-19.9069361287402\\
13.7414375726169	-20.845071279026\\
12.390786354824	-21.7020507839214\\
10.9884186099222	-22.4744518587606\\
9.539802805115	-23.1591673663677\\
8.05059424764734	-23.7534178160121\\
6.52661393886862	-24.2547621981871\\
4.97382677874819	-24.6611076147665\\
3.39831919848018	-24.9707176681119\\
1.80627630099459	-25.1822195768551\\
0.203958591105259	-25.2946099903504\\
-1.40232162133624	-25.3072594781648\\
-3.00622406055315	-25.2199156754403\\
-4.60140448042301	-25.0327050695124\\
-6.18153872994331	-24.7461334177739\\
-7.74034680151477	-24.361084791436\\
-9.27161677478415	-23.8788192445347\\
-10.7692285688968	-23.3009691122432\\
-12.2271774164171	-22.6295339472778\\
-13.6395969728828	-21.8668741078918\\
-15.0007819769659	-21.0157030156456\\
-16.3052103775127	-20.0790781057854\\
-17.547564845336	-19.0603904976578\\
-18.7227535895122	-17.9633534171152\\
-19.8259304001101	-16.7919894072994\\
-20.8525138417249	-15.5506163685385\\
-21.7982055249103	-14.2438324723113\\
-22.6590073855893	-12.876499998336\\
-23.4312379057593	-11.4537281477911\\
-24.1115472122997	-9.98085488947718\\
-24.6969309944064	-8.46342789935526\\
-25.184743184128	-6.90718465734579\\
-25.572707348635	-5.31803176852082\\
-25.8589267472153	-3.70202357886817\\
-26.0418930105311	-2.06534015862959\\
-26.1204934043923	-0.414264728812728\\
-26.0940166451739	1.24483939116882\\
-25.962157239024	2.9055522346649\\
-25.7250183221464	4.56142095585715\\
-25.3831129846969	6.20598383123271\\
-24.937364066172	7.83279440966106\\
-24.389102415585	9.43544572524272\\
-23.7400636152001	11.0075944863554\\
-22.9923831721028	12.5429851538712\\
-22.1485901874159	14.0354738213605\\
-21.2115995185032	15.4790518102384\\
-20.1847024550105	16.8678688932486\\
-19.0715559350737	18.1962560604224\\
-17.8761703334368	19.458747742689\\
-16.6028958585689	20.6501034096595\\
-15.2564076011158	21.7653284597434\\
-13.8416892811527	22.799694322698\\
-12.3640157467135	23.7487576969324\\
-10.8289342809151	24.6083788464121\\
-9.24224477968476	25.3747388847977\\
-7.6099788665901	26.0443559775299\\
-5.9383780155677	26.6141003959054\\
-4.23387075641616	27.0812083607882\\
-2.50304904175807	27.4432946174401\\
-0.752643857759823	27.6983636870387\\
1.01049983578339	27.8448197447571\\
2.77944874735101	27.8814750787974\\
4.54720738619748	27.8075570894927\\
6.30674459161834	27.6227137924952\\
8.05102036302776	27.3270177951451\\
9.77301289309804	26.9209687203448\\
11.4657457047514	26.4054940576319\\
13.1223147916811	25.7819484266327\\
14.7359156613139	25.0521112436727\\
16.2998701787245	24.2181827879957\\
17.8076531099657	23.2827786697902\\
19.252918263605	22.2489227080037\\
20.6295241299491	21.1200382317529\\
21.931558918499	19.8999378249499\\
23.1533648956091	18.5928115395818\\
24.2895619261236	17.2032136088501\\
25.335070124924	15.7360476970991\\
26.2851315268487	14.1965507291033\\
27.1353306863226	12.5902753468341\\
27.8816141212614	10.9230710472499\\
28.5203085193872	9.20106405994886\\
29.048137628986	7.43063602865342\\
29.4622377603599	5.61840156545116\\
29.76017182875	3.77118475146936\\
29.9399418743343	1.89599466220109\\
30	-0\\
};
\addplot [color=red, line width=1.5pt, forget plot]
  table[row sep=crcr]{%
30	0\\
29.9848952395501	-0.950909126674481\\
29.9396567950611	-1.89905361088759\\
29.8643869184689	-2.84351969918574\\
29.7592167754245	-3.78339897216333\\
29.6243062627484	-4.71778917971259\\
29.4598437994961	-5.64579506874857\\
29.2660460918867	-6.56652920269036\\
29.043157872368	-7.479112771989\\
28.7914516131107	-8.38267639500198\\
28.5112272142519	-9.27636090852516\\
28.2028116672259	-10.159318147303\\
27.866558693541	-11.0307117118499\\
27.5028483593875	-11.8897177239274\\
27.1120866664745	-12.7355255690341\\
26.6947051195201	-13.5673386252781\\
26.2511602708379	-14.3843749780159\\
25.7819332424779	-15.1858681196542\\
25.2875292264051	-15.9710676340273\\
24.7684769632127	-16.7392398647753\\
24.2253281998863	-17.4896685671663\\
23.6586571271559	-18.2216555428192\\
23.069059796982	-18.9345212567998\\
22.4571535207472	-19.6276054365826\\
21.823576248736	-20.3002676523823\\
21.1689859314995	-20.9518878783812\\
20.494059863721	-21.5818670343934\\
19.7994940112091	-22.1896275075255\\
19.0860023216599	-22.774613653412\\
18.3543160198435	-23.3362922766203\\
17.6051828878808	-23.8741530898431\\
16.8393665312914	-24.3877091515111\\
16.057645631501	-24.8764972814779\\
15.260813185511	-25.3400784544555\\
14.4496757334401	-25.7780381708869\\
13.6250525746589	-26.1899868049752\\
12.7877749732476	-26.575559929598\\
11.938685353512	-26.9344186178637\\
11.0786364863053	-27.2662497210825\\
10.2084906669061	-27.5707661229477\\
9.32911888520954	-27.8477069697435\\
8.44139998899761	-28.0968378764156\\
7.54621984105442	-28.3179511083617\\
6.6444704708999	-28.5108657388229\\
5.73704922191821	-28.675427781773\\
4.82485789465883	-28.8115103002299\\
3.90880188709193	-28.9190134899295\\
2.98978933260015	-28.9978647383259\\
2.06873023649017	-29.0480186589037\\
1.14653561180738	-29.0694571008066\\
0.224116615236712	-29.0621891338112\\
-0.697616316128888	-29.0262510086923\\
-1.61775432637225	-28.9617060930503\\
-2.53539099991097	-28.8686447826895\\
-3.44962321745727	-28.7471843886582\\
-4.35955200800855	-28.5974690000819\\
-5.26428339610278	-28.419669322942\\
-6.162929243578	-28.2139824949712\\
-7.0546080850812	-27.9806318768579\\
-7.93844595657799	-27.7198668199721\\
-8.81357721612181	-27.4319624108456\\
-9.67914535614833	-27.1172191926558\\
-10.5343038065707	-26.7759628639862\\
-11.378216727958	-26.4085439551517\\
-12.2100597940901	-26.0153374823982\\
-13.0290209631929	-25.5967425803038\\
-13.8343012371659	-25.1531821127249\\
-14.6251154081284	-24.6851022626533\\
-15.4006927916207	-24.1929721013632\\
-16.1602779458088	-23.6772831372451\\
-16.903131376056	-23.1385488447448\\
-17.6285302242352	-22.5773041738348\\
-18.3357689421714	-21.9941050404685\\
-19.0241599486203	-21.3895277984794\\
-19.693034269199	-20.7641686934036\\
-20.3417421587047	-20.1186432987202\\
-20.9696537052702	-19.4535859350153\\
-21.576159415825	-18.769649072596\\
-22.1606707823414	-18.0675027180864\\
-22.7226208283702	-17.3478337855556\\
-23.2614646353809	-16.6113454527407\\
-23.7766798484439	-15.8587565029384\\
-24.267767160809	-15.0908006531501\\
-24.7342507769538	-14.3082258690787\\
-25.1756788536927	-13.5117936675849\\
-25.5916239189614	-12.7022784072213\\
-25.981683267905	-11.8804665674721\\
-26.3454793359242	-11.0471560173362\\
-26.6826600483505	-10.2031552738991\\
-26.9928991464427	-9.34928275154912\\
-27.2758964894185	-8.4863660024987\\
-27.531378332258	-7.61524094928034\\
-27.7590975790304	-6.73675110989345\\
-27.9588340115274	-5.85174681628254\\
-28.1303944929972	-4.96108442683516\\
-28.2736131468043	-4.06562553359095\\
-28.3883515098562	-3.16623616485829\\
-28.4744986606616	-2.26378598393898\\
-28.5319713219122	-1.35914748466375\\
-28.5607139374916	-0.453195184444992\\
-28.560698723849	0.453195184445464\\
-28.5319256956903	1.35914748466423\\
-28.4744226659642	2.26378598393946\\
-28.3882452201445	3.16623616485876\\
-28.2734766648293	4.0656255335914\\
-28.1302279507037	4.96108442683564\\
-27.9586375699327	5.85174681628304\\
-27.7588714280755	6.73675110989398\\
-27.5311226906312	7.61524094928086\\
-27.275611604354	8.48636600249921\\
-26.9925852934907	9.34928275154971\\
-26.6823175311236	10.2031552738998\\
-26.3451084858152	11.0471560173368\\
-25.9812844437809	11.8804665674727\\
-25.591197506831	12.7022784072218\\
-25.175225266349	13.5117936675853\\
-24.7337704535913	14.3082258690792\\
-24.2672605666179	15.0908006531507\\
-23.7761474741777	15.858756502939\\
-23.2609069969025	16.6113454527413\\
-22.7220384661731	17.3478337855561\\
-22.1600642610483	18.067502718087\\
-21.5755293236642	18.7696490725966\\
-20.9690006535296	19.4535859350158\\
-20.3410667811641	20.1186432987207\\
-19.6923372215414	20.7641686934044\\
-19.0234419078227	21.3895277984801\\
-18.3350306058756	21.9941050404691\\
-17.6277723100985	22.5773041738353\\
-16.9023546210841	23.1385488447454\\
-16.1594831056689	23.6772831372457\\
-15.3998806399384	24.1929721013638\\
-14.6242867357666	24.685102262654\\
-13.8334568514871	25.1531821127254\\
-13.0281616873064	25.5967425803044\\
-12.2091864660833	26.0153374823987\\
-11.3773302001137	26.4085439551521\\
-10.5334049445708	26.7759628639866\\
-9.67823503826363	27.1172191926565\\
-8.81265633239037	27.4319624108463\\
-7.93751540797157	27.7198668199727\\
-7.05366878266064	27.9806318768586\\
-6.1619821076388	28.2139824949719\\
-5.26332935531109	28.4196693229426\\
-4.35859199852868	28.5974690000824\\
-3.44865818207137	28.7471843886586\\
-2.53442188713171	28.8686447826899\\
-1.6167820895494	28.9617060930507\\
-0.696641912550259	29.0262510086926\\
0.225092225248714	29.0621891338115\\
1.14751146580314	29.0694571008067\\
2.06970537080309	29.0480186589036\\
2.99076278325918	28.9978647383256\\
3.90977269073537	28.9190134899291\\
4.82582508944855	28.8115103002297\\
5.73801184845374	28.675427781773\\
6.64542757313121	28.510865738823\\
7.54717046719248	28.3179511083618\\
8.44234319242289	28.0968378764157\\
9.33005372537611	27.8477069697434\\
10.2094162102416	27.5707661229477\\
11.0795518071057	27.2662497210826\\
11.9395895348299	26.9344186178639\\
12.7886671077741	26.5755599295981\\
13.6259317655977	26.1899868049753\\
14.450541095372	25.7780381708869\\
15.2616638452508	25.3400784544555\\
16.0584807289434	24.8764972814779\\
16.8401852202455	24.3877091515111\\
17.6059843368936	23.8741530898433\\
18.3550994130108	23.3362922766202\\
19.0867668594243	22.774613653412\\
19.8002389111429	22.1896275075255\\
20.4947843612963	21.5818670343934\\
21.169689280841	20.9518878783812\\
21.8242577233586	20.3002676523824\\
22.457812414277	19.6276054365826\\
23.069695423859	18.9345212567998\\
23.6592688233193	18.2216555428191\\
24.2259153234401	17.4896685671662\\
24.7690388950731	16.7392398647752\\
25.2880653709269	15.9710676340272\\
25.7824430280593	15.1858681196543\\
26.2516431505062	14.384374978016\\
26.6951605714939	13.5673386252783\\
27.1125141947036	12.7355255690341\\
27.5032474940708	11.8897177239274\\
27.8669289916196	11.0307117118499\\
28.2031527128527	10.1593181473031\\
28.5115386192376	9.27636090852518\\
28.7917330173432	8.38267639500197\\
29.0434089442084	7.47911277198903\\
29.2662665285377	6.56652920269035\\
29.4600333273453	5.64579506874855\\
29.624464637685	4.71778917971258\\
29.7593437831288	3.78339897216333\\
29.8644823746742	2.84351969918574\\
29.9397205457895	1.89905361088758\\
29.9849271613185	0.950909126674478\\
30	-0\\
};
\end{axis}

\end{tikzpicture}%
